Practical Parallel Algorithms for Near-Optimal Densest Subgraphs on Massive Graphs

The densest subgraph problem has received significant attention, both in theory and in practice, due to its applications in problems such as community detection, social network analysis, and spam detection. Due to the high cost of obtaining exact solutions, much attention has focused on designing approximate densest subgraph algorithms. However, existing approaches are not able to scale to massive graphs with billions of edges. In this paper, we introduce a new framework that combines approximate densest subgraph algorithms with a pruning optimization. We design new parallel variants of the state-of-the-art sequential Greedy++ algorithm, and plug it into our framework in conjunction with a parallel pruning technique based on $k$-core decomposition to obtain parallel $(1+\varepsilon)$-approximate densest subgraph algorithms. On a single thread, our algorithms achieve $2.6$--$34\times$ speedup over Greedy++, and obtain up to $22.37\times$ self relative parallel speedup on a 30-core machine with two-way hyper-threading. Compared with the state-of-the-art parallel algorithm by Harb et al. [NeurIPS'22], we achieve up to a $114\times$ speedup on the same machine. Finally, against the recent sequential algorithm of Xu et al. [PACMMOD'23], we achieve up to a $25.9\times$ speedup. The scalability of our algorithms enables us to obtain near-optimal density statistics on the hyperlink2012 (with roughly 113 billion edges) and clueweb (with roughly 37 billion edges) graphs for the first time in the literature.

==> combine.tex <==
\section{Parallel Algorithms with Pruning}


\begin{algorithm}[t!]\caption{\PGreedySortingPP\ with pruning}\label{alg:sortingpp_prune}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwFor{For}{for}{do}{endfor}
    \SetKw{KwIn}{in}
    \SetKw{KwLet}{let}
    \SetKwFor{ParFor}{parfor}{do}{endparfor}

    \DontPrintSemicolon
    
    \Input{an input graph $G=(V,E)$, number of iterations $T$}
    \Output{density of approximate densest subgraph found}
    \SetAlgoVlined
    $cores, k_{max} := Coreness(G)$ \;
    $\rho_{max} \leftarrow k_{max}/2$\;
    $G \leftarrow core(G,k_{max}/2)$ \julian{do we need to take the ceiling here}\;
    $S \leftarrow G$\;
    \ParFor{v \KwIn V}{
        $\ell(v) \leftarrow 0$ \;
    }

    \For{i=1 \KwTo T}{
        \KwLet $v_1, \ldots, v_n$ be such that $\ell(v_1) \leq \ell(v_2) \leq \ldots \leq \ell(v_n)$\;
        $\ell, \rho := PeelWithOrdering(G,v_1\ldots v_n, \ell)$\;
        \If{$\lceil\rho\rceil> \lceil\rho_{max} \rceil$}{
            $\rho_{max} \leftarrow \rho$\;
            $G \leftarrow core(G, \lceil \rho_{max} \rceil)$ \tcp*[l]{using $cores$ from Line 1}
        }
    }
    \Return{$\rho_{max}$}
        
\end{algorithm}


In this section, we combine the pruning idea in \cref{sec:pruning} and parallel algorithms in \cref{sec:algo}. This results in an algorithm that works much better in practice.
The pseudocode of our algorithm is shown in \cref{alg:sortingpp_prune}. \julian{i'm not sure we need the pseudocode of \cref{alg:sortingpp_prune} as we already defined the framework and this algorithm is an instantiation of the framework}
We first compute core numbers of vertices in the graph using the algorithm of Dhulipala et al.~\cite{dhulipala2017julienne} (Line 1). We then shrink the graph to $core(G,\lceil k_{max}/2 \rceil)$ (Line 3). The initialization of loads is done in parallel (Lines 5--6).
Then, for each iteration, we obtain an ordering: either a degeneracy ordering (\GreedyPP) or a sorted ordering (\GreedySortingPP) (Line 8). We then call~\cref{alg:peel_ordering} with the ordering (Line 9). Next, we update the density and further shrink the graph to $core(G, \lceil \rho_{max} \rceil)$, where $\rho_{max}$ is the maximum density found so far (Lines 10--12).
\julian{The computation on Line 12 can use the core numbers already computed on Line 1, since core numbers of vertices do not change even after pruning.}
Finally, we return the densest subgraph found throughout $T$ iterations (Line 13). Although the algorithm in \cref{alg:sortingpp_prune} returns only the value of the approximate densest subgraph found, we could turn it into an algorithm that returns an actual approximate densest subgraph by recording the time step on which the best density was found and running the algorithm again until that specific time step to obtain the graph. 

Combining approximate $k$-core for pruning with \PGreedySortingPP\ gives


This algorithm has $O(T(n+m))$ total work and $O(T \log n + \rho \log n)$ total depth. 

\julian{check bounds based on earlier comments} 
Note that while pruning gives speedups in practice, it does not 
improve the theoretical complexity of the algorithm, as there exists graph where the core that we prune down to covers most of the original graph. As an example, the maximum non-empty core of a clique is the clique itself.



\julian{since this is a non-theory conference, it is good to have figures showing how our algorithm works on a small example. here are some suggested figures:  1) example illustrating how the graph gets pruned over time using Algorithm 4; if we have space
2) example illustrating peeling to completion of Greedy++ vs. GreedySorting++, showing how the loads change on each iteration.

}
